Fermi-LAT counterparts of IceCube neutrinos above 100 TeV

The IceCube Collaboration has published four years of data and the observed neutrino flux is significantly in excess of the expected atmospheric background. Due to the steeply falling atmospheric background spectrum, events at the highest energies are most likely extraterrestrial. In our previous approach we have studied blazars as the possible origin of the High-Energy Starting Events (HESE) neutrino events at PeV energies. In this work we extend our study to include all HESE neutrinos (which does not include IC 170922A) at or above a reconstructed energy of 100 TeV, but below 1 PeV. We study the X-ray and $\gamma$-ray data of all ($\sim200$) 3LAC blazars that are positionally consistent with the neutrino events above 100 TeV to determine the maximum neutrino flux from these sources. This larger sample allows us to better constrain the scaling factor between the observed and maximum number of neutrino events. We find that when we consider a realistic neutrino spectrum and other factors, the number of neutrinos is in good agreement with the detected number of IceCube HESE events. We also show that there is no direct correlation between \Fermi-LAT $\gamma$-ray flux and the IceCube neutrino flux and that the expected number of neutrinos is consistent with the non-detection of individual bright blazars.

==> nunum.tex <==
\begin{table}[b]\centering\fontsize{5.5}{5.7}\selectfont
\caption{Neutrino numbers for all sources. This table lists the IceCube HESE event number in the first column, the maximum number of neutrinos in the second column, the neutrino number scaled to the empirical factor in the third column, and the neutrino numbers corrected for the realistic neutrino spectrum in the fourth column, integrated over the full energy range (which does not take into account that other neutrinos may have been seen from a given source).The last column shows the values with the blazar and neutrino flavor scalings applied. Within each neutrino event sources are ordered by their predicted number of neutrinos. Neutrinos from sources that appear multiple times, because of overlap of their uncertainty regions, are marked with parentheses the second time, and only the first of their neutrino expectations are counted.}
\label{tab-nunum}
\begin{tabular}{llllll}

IC & Source & \#$\nu$ & \#$\nu_{\mathrm{emp.}}$ & \#$\nu_{\mathrm{scale, int.}}$ & \#$\nu_{\mathrm{f}}$\\
\hline
2 & PKS1830-211 & 50.18 & 4.47e-01 & 1.07e+01 & 2.68e+00\\
 & 1RXSJ174459.5-172640 & 21.10 & 1.88e-01 & 4.51e+00 & 1.13e+00\\
 & SwiftJ1656.3-3302 & 17.14 & 1.53e-01 & 3.66e+00 & 9.15e-01\\
 & 1RXSJ182853.8-241746 & 16.52 & 1.47e-01 & 3.53e+00 & 8.82e-01\\
 & TXS1714-336 & 13.48 & 1.20e-01 & 2.88e+00 & 7.19e-01\\
 & PMNJ1802-3940 & 8.90 & 7.92e-02 & 1.90e+00 & 4.75e-01\\
 & PKS1730-13 & 6.33 & 5.64e-02 & 1.35e+00 & 3.38e-01\\
 & PKSB1908-201 & 6.22 & 5.53e-02 & 1.33e+00 & 3.32e-01\\
 & PKSB1921-293 & 5.24 & 4.66e-02 & 1.12e+00 & 2.80e-01\\
 & PKS1954-388 & 4.99 & 4.45e-02 & 1.07e+00 & 2.67e-01\\
 & PKS1933-400 & 4.93 & 4.39e-02 & 1.05e+00 & 2.63e-01\\
 & TXS1920-211 & 3.84 & 3.42e-02 & 8.20e-01 & 2.05e-01\\
 & PMNJ1912-0804 & 2.80 & 2.50e-02 & 5.99e-01 & 1.50e-01\\
 & PMNJ2000-2931 & 2.56 & 2.28e-02 & 5.47e-01 & 1.37e-01\\
 & 1RXSJ171405.2-202747 & 2.56 & 2.28e-02 & 5.46e-01 & 1.37e-01\\
 & PMNJ1959-4246 & 2.54 & 2.26e-02 & 5.42e-01 & 1.36e-01\\
 & PMNJ1936-4719 & 2.52 & 2.24e-02 & 5.38e-01 & 1.35e-01\\
 & PMNJ1858-2511 & 2.49 & 2.22e-02 & 5.33e-01 & 1.33e-01\\
 & TXS1951-115 & 2.33 & 2.07e-02 & 4.98e-01 & 1.24e-01\\
 & PMNJ1758-4820 & 2.20 & 1.96e-02 & 4.70e-01 & 1.17e-01\\
 & PMNJ1718-3056 & 2.10 & 1.87e-02 & 4.49e-01 & 1.12e-01\\
 & PKS1958-179 & 2.08 & 1.85e-02 & 4.44e-01 & 1.11e-01\\
 & TXS2002-233 & 1.99 & 1.77e-02 & 4.24e-01 & 1.06e-01\\
 & 1RXSJ195815.6-301119 & 1.95 & 1.74e-02 & 4.17e-01 & 1.04e-01\\
 & PKS1929-457 & 1.94 & 1.73e-02 & 4.14e-01 & 1.04e-01\\
 & PKS2021-330 & 1.92 & 1.71e-02 & 4.09e-01 & 1.02e-01\\
 & 1RXSJ184919.7-164726 & 1.89 & 1.68e-02 & 4.04e-01 & 1.01e-01\\
 & TXS1909-124 & 1.58 & 1.41e-02 & 3.37e-01 & 8.43e-02\\
 & PKS2005-489 & 1.50 & 1.34e-02 & 3.21e-01 & 8.03e-02\\
 & PMNJ1830-4441 & 1.49 & 1.32e-02 & 3.18e-01 & 7.94e-02\\
 & NVSSJ165949-313047 & 1.43 & 1.27e-02 & 3.06e-01 & 7.64e-02\\
 & PMNJ1735-1117 & 1.43 & 1.27e-02 & 3.04e-01 & 7.61e-02\\
 & PKS1821-525 & 1.41 & 1.26e-02 & 3.02e-01 & 7.55e-02\\
 & NVSSJ173146-300309 & 1.37 & 1.22e-02 & 2.92e-01 & 7.30e-02\\
 & 1RXSJ194306.8-351001 & 1.33 & 1.19e-02 & 2.84e-01 & 7.11e-02\\
 & 1H1914-194 & 1.29 & 1.15e-02 & 2.76e-01 & 6.89e-02\\
 & PKS1942-313 & 1.19 & 1.06e-02 & 2.55e-01 & 6.37e-02\\
 & NVSSJ174154-253743 & 1.18 & 1.05e-02 & 2.52e-01 & 6.29e-02\\
 & PMNJ1911-1908 & 1.16 & 1.04e-02 & 2.48e-01 & 6.21e-02\\
 & 1RXSJ195500.6-160328 & 1.10 & 9.80e-03 & 2.35e-01 & 5.88e-02\\
 & PKS2004-447 & 1.09 & 9.67e-03 & 2.32e-01 & 5.80e-02\\
 & PMNJ1918-4111 & 1.08 & 9.63e-03 & 2.31e-01 & 5.78e-02\\
 & NVSSJ182338-345412 & 0.98 & 8.75e-03 & 2.10e-01 & 5.25e-02\\
 & PMNJ1808-5011 & 0.83 & 7.39e-03 & 1.77e-01 & 4.43e-02\\
 & PMNJ1849-4314 & 0.79 & 7.00e-03 & 1.68e-01 & 4.20e-02\\
 & PMNJ1921-1607 & 0.78 & 6.94e-03 & 1.67e-01 & 4.16e-02\\
 & SUMSSJ195945-472519 & 0.77 & 6.89e-03 & 1.65e-01 & 4.13e-02\\
 & PMNJ1753-5015 & 0.76 & 6.75e-03 & 1.62e-01 & 4.05e-02\\
 & PMNJ1831-2714 & 0.76 & 6.74e-03 & 1.62e-01 & 4.04e-02\\
 & PMNJ2036-2830 & 0.64 & 5.73e-03 & 1.37e-01 & 3.43e-02\\
 & PMNJ1816-4943 & 0.62 & 5.54e-03 & 1.33e-01 & 3.32e-02\\
 & PMNJ2012-1646 & 0.60 & 5.38e-03 & 1.29e-01 & 3.22e-02\\
 & TXS1918-126 & 0.60 & 5.37e-03 & 1.29e-01 & 3.22e-02\\
 & NVSSJ204150-373341 & 0.47 & 4.22e-03 & 1.01e-01 & 2.53e-02\\
 & PMNJ2022-4513 & 0.44 & 3.94e-03 & 9.45e-02 & 2.36e-02\\
 & PKS1953-325 & 0.41 & 3.66e-03 & 8.77e-02 & 2.19e-02\\
 & 1RXSJ201731.2-411452 & 0.39 & 3.50e-03 & 8.40e-02 & 2.10e-02\\
 & 1RXSJ203650.9-332817 & 0.37 & 3.31e-03 & 7.93e-02 & 1.98e-02\\
 & PMNJ1913-3630 & 0.32 & 2.84e-03 & 6.82e-02 & 1.71e-02\\
 & PMNJ1848-4230 & 0.20 & 1.82e-03 & 4.36e-02 & 1.09e-02\\
 & SUMSSJ193946-492539 & 0.15 & 1.35e-03 & 3.23e-02 & 8.09e-03\\
 & 1RXSJ194422.6-452326 & 0.10 & 8.58e-04 & 2.06e-02 & 5.15e-03\\
\hline
& & \textbf{223.40} & \textbf{2.0e+00} &\textbf{47.7}  & \textbf{1.2e+01} \\
\hline
\end{tabular}
\end{table}
\begin{table}[b]\centering\fontsize{5.5}{5.7}\selectfont
\addtocounter{table}{-1}
\caption{contd.}
\begin{tabular}{llllll}

IC & Source & \#$\nu$ & \#$\nu_{\mathrm{emp.}}$ & \#$\nu_{\mathrm{scale, int.}}$ & \#$\nu_{\mathrm{f}}$\\
\hline
4 & MRC1036-529 & 7.02 & 6.24e-02 & 1.29e+00 & 3.22e-01\\
 & PKS1116-46 & 3.42 & 3.05e-02 & 6.29e-01 & 1.57e-01\\
 & PKS1101-536 & 3.40 & 3.02e-02 & 6.24e-01 & 1.56e-01\\
 & PKS1104-445 & 3.03 & 2.70e-02 & 5.57e-01 & 1.39e-01\\
 & PMNJ1109-4815 & 1.64 & 1.46e-02 & 3.02e-01 & 7.56e-02\\
\hline
& & \textbf{18.51} & \textbf{1.6e-01} &\textbf{3.4}  & \textbf{8.5e-01} \\
\hline
12 & PMNJ1936-4719 & 2.83 & 2.52e-02 & 5.38e-01 & 1.35e-01\\
 & (PKS1936-623) & 2.71 & 2.42e-02 & 5.16e-01 & 1.29e-01\\
 & PKS1929-457 & 2.35 & 2.09e-02 & 4.46e-01 & 1.12e-01\\
 & PKS2005-489 & 1.69 & 1.51e-02 & 3.21e-01 & 8.03e-02\\
 & (PKS2004-447) & 1.22 & 1.09e-02 & 2.32e-01 & 5.80e-02\\
 & PMNJ1949-6137 & 0.94 & 8.39e-03 & 1.79e-01 & 4.48e-02\\
 & (SUMSSJ195945-472519) & 0.87 & 7.74e-03 & 1.65e-01 & 4.13e-02\\
 & (1RXSJ195503.1-564031) & 0.64 & 5.67e-03 & 1.21e-01 & 3.03e-02\\
 & (PKS2036-577) & 0.57 & 5.08e-03 & 1.08e-01 & 2.71e-02\\
 & (PMNJ2022-4513) & 0.50 & 4.43e-03 & 9.45e-02 & 2.36e-02\\
 & (SUMSSJ193946-492539) & 0.17 & 1.52e-03 & 3.23e-02 & 8.09e-03\\
 & (1RXSJ194422.6-452326) & 0.11 & 9.64e-04 & 2.06e-02 & 5.15e-03\\
\hline
& & \textbf{14.61} & \textbf{1.3e-01} &\textbf{2.8}  & \textbf{6.9e-01} \\
\hline
13& NONE & 0.0 & 0.0 & 0.0\\
\hline
& & \textbf{0.00} & \textbf{0.0e+00} &\textbf{0.0}  & \textbf{0.0e+00} \\
\hline
17 & PG1553+113 & 7.15 & 6.36e-02 & 1.26e+00 & 3.14e-01\\
 & 1RXSJ163717.1+131418 & 5.31 & 4.73e-02 & 9.33e-01 & 2.33e-01\\
 & 4C+10.45 & 2.16 & 1.93e-02 & 3.80e-01 & 9.50e-02\\
 & 4C+15.54 & 1.57 & 1.40e-02 & 2.76e-01 & 6.91e-02\\
 & PKS1551+130 & 1.53 & 1.36e-02 & 2.69e-01 & 6.73e-02\\
 & MG1J163119+1051 & 1.33 & 1.18e-02 & 2.33e-01 & 5.84e-02\\
 & MG1J165034+0824 & 1.33 & 1.18e-02 & 2.33e-01 & 5.84e-02\\
 & 1ES1552+203 & 0.91 & 8.13e-03 & 1.60e-01 & 4.01e-02\\
 & MG2J165546+2043 & 0.68 & 6.06e-03 & 1.20e-01 & 2.99e-02\\
 & MG1J154930+1708 & 0.50 & 4.41e-03 & 8.70e-02 & 2.17e-02\\
 & TXS1549+089 & 0.31 & 2.80e-03 & 5.53e-02 & 1.38e-02\\
 & MG1J160340+1106 & 0.26 & 2.32e-03 & 4.59e-02 & 1.15e-02\\
 & 87GB155744.0+232525 & 0.26 & 2.27e-03 & 4.48e-02 & 1.12e-02\\
 & TXS1638+118 & 0.21 & 1.88e-03 & 3.71e-02 & 9.28e-03\\
 & MG1J154628+1817 & 0.11 & 1.02e-03 & 2.02e-02 & 5.05e-03\\
\hline
& & \textbf{23.64} & \textbf{2.1e-01} &\textbf{4.2}  & \textbf{1.0e+00} \\
\hline
22 & (PKSB1908-201) & 7.57 & 6.74e-02 & 1.33e+00 & 3.32e-01\\
 & (PKSB1921-293) & 7.21 & 6.42e-02 & 1.26e+00 & 3.16e-01\\
 & (TXS1920-211) & 4.68 & 4.16e-02 & 8.20e-01 & 2.05e-01\\
 & (PMNJ2000-2931) & 3.26 & 2.90e-02 & 5.72e-01 & 1.43e-01\\
 & (PMNJ1858-2511) & 3.04 & 2.71e-02 & 5.33e-01 & 1.33e-01\\
 & (TXS1951-115) & 2.84 & 2.53e-02 & 4.98e-01 & 1.24e-01\\
 & (PKS1958-179) & 2.71 & 2.41e-02 & 4.75e-01 & 1.19e-01\\
 & (TXS2002-233) & 2.42 & 2.15e-02 & 4.24e-01 & 1.06e-01\\
 & (1RXSJ195815.6-301119) & 2.38 & 2.12e-02 & 4.17e-01 & 1.04e-01\\
 & (1RXSJ184919.7-164726) & 2.30 & 2.05e-02 & 4.04e-01 & 1.01e-01\\
 & (TXS1909-124) & 1.92 & 1.71e-02 & 3.37e-01 & 8.43e-02\\
 & (1H1914-194) & 1.57 & 1.40e-02 & 2.76e-01 & 6.89e-02\\
 & (PKS1942-313) & 1.45 & 1.29e-02 & 2.55e-01 & 6.37e-02\\
 & (PMNJ1911-1908) & 1.42 & 1.26e-02 & 2.48e-01 & 6.21e-02\\
 & (PMNJ1921-1607) & 0.95 & 8.46e-03 & 1.67e-01 & 4.16e-02\\
 & (1RXSJ195500.6-160328) & 0.89 & 7.94e-03 & 1.56e-01 & 3.91e-02\\
 & (PMNJ2012-1646) & 0.74 & 6.55e-03 & 1.29e-01 & 3.22e-02\\
 & (TXS1918-126) & 0.73 & 6.52e-03 & 1.28e-01 & 3.21e-02\\
 & (PKS1953-325) & 0.50 & 4.45e-03 & 8.77e-02 & 2.19e-02\\
\hline
& & \textbf{48.59} & \textbf{4.3e-01} &\textbf{8.5}  & \textbf{2.1e+00} \\
\hline
\end{tabular}
\end{table}
\begin{table}[b]\centering\fontsize{5.5}{5.7}\selectfont
\addtocounter{table}{-1}
\caption{contd.}
\begin{tabular}{llllll}

IC & Source & \#$\nu$ & \#$\nu_{\mathrm{emp.}}$ & \#$\nu_{\mathrm{scale, int.}}$ & \#$\nu_{\mathrm{f}}$\\
\hline
26 & RXJ0959.4+2123 & 6.24 & 5.55e-02 & 1.01e+00 & 2.52e-01\\
 & OJ287 & 2.66 & 2.37e-02 & 4.31e-01 & 1.08e-01\\
 & MG2J101241+2439 & 1.96 & 1.74e-02 & 3.17e-01 & 7.92e-02\\
 & 1RXSJ091211.9+275955 & 1.54 & 1.37e-02 & 2.49e-01 & 6.21e-02\\
 & OK290 & 1.21 & 1.07e-02 & 1.95e-01 & 4.89e-02\\
 & TXS0907+230 & 1.13 & 1.01e-02 & 1.83e-01 & 4.57e-02\\
 & 1RXSJ100235.8+221609 & 1.12 & 1.00e-02 & 1.82e-01 & 4.55e-02\\
 & GB6J0905+2748A & 1.08 & 9.63e-03 & 1.75e-01 & 4.38e-02\\
 & MG2J094148+2728 & 1.00 & 8.91e-03 & 1.62e-01 & 4.05e-02\\
 & Ton0396 & 0.90 & 7.99e-03 & 1.45e-01 & 3.63e-02\\
 & B20920+28 & 0.84 & 7.51e-03 & 1.37e-01 & 3.41e-02\\
 & SDSSJ091230.61+155528.0 & 0.68 & 6.07e-03 & 1.10e-01 & 2.76e-02\\
 & GB6J1001+2911 & 0.68 & 6.05e-03 & 1.10e-01 & 2.75e-02\\
 & MG1J090534+1358 & 0.48 & 4.23e-03 & 7.69e-02 & 1.92e-02\\
 & NVSSJ090226+205045 & 0.43 & 3.84e-03 & 6.99e-02 & 1.75e-02\\
 & TXS0853+211 & 0.25 & 2.26e-03 & 4.11e-02 & 1.03e-02\\
 & PKS1000+26 & 0.25 & 2.22e-03 & 4.04e-02 & 1.01e-02\\
 & NVSSJ101808+190614 & 0.24 & 2.18e-03 & 3.96e-02 & 9.90e-03\\
 & MG1J101810+1903 & 0.24 & 2.18e-03 & 3.96e-02 & 9.90e-03\\
 & RXJ0908.9+2311 & 0.21 & 1.86e-03 & 3.39e-02 & 8.48e-03\\
 & B20922+31B & 0.08 & 7.49e-04 & 1.36e-02 & 3.41e-03\\
\hline
& & \textbf{23.23} & \textbf{2.1e-01} &\textbf{3.8}  & \textbf{9.4e-01} \\
\hline
30 & PKS0637-75 & 5.75 & 5.12e-02 & 1.03e+00 & 2.59e-01\\
 & PMNJ0251-8226 & 4.21 & 3.75e-02 & 7.57e-01 & 1.89e-01\\
 & SUMSSJ054923-874001 & 3.89 & 3.46e-02 & 6.99e-01 & 1.75e-01\\
 & PKS0736-770 & 1.45 & 1.29e-02 & 2.61e-01 & 6.53e-02\\
 & PMNJ0810-7530 & 1.36 & 1.21e-02 & 2.44e-01 & 6.11e-02\\
 & PKS0541-834 & 0.95 & 8.43e-03 & 1.70e-01 & 4.26e-02\\
 & PKS1029-85 & 0.82 & 7.28e-03 & 1.47e-01 & 3.68e-02\\
 & SUMSSJ074220-813139 & 0.00 & 0.00e+00 & 0.00e+00 & 0.00e+00\\
\hline
& & \textbf{18.43} & \textbf{1.6e-01} &\textbf{3.3}  & \textbf{8.3e-01} \\
\hline
33 & NVSSJ195547+021514 & 5.14 & 4.57e-02 & 1.20e+00 & 2.99e-01\\
 & RXJ1931.1+0937 & 2.72 & 2.42e-02 & 6.35e-01 & 1.59e-01\\
 & 1RXSJ194246.3+103339 & 1.69 & 1.51e-02 & 3.94e-01 & 9.86e-02\\
 & NVSSJ201431+064849 & 1.60 & 1.42e-02 & 3.73e-01 & 9.32e-02\\
 & TXS1923+123 & 0.94 & 8.33e-03 & 2.18e-01 & 5.45e-02\\
 & 1RXSJ193320.3+072616 & 0.75 & 6.63e-03 & 1.74e-01 & 4.34e-02\\
 & 87GB195252.4+135009 & 0.69 & 6.11e-03 & 1.60e-01 & 4.00e-02\\
 & NVSSJ190836-012642 & 0.45 & 3.99e-03 & 1.04e-01 & 2.61e-02\\
 & PMNJ2014-0047 & 0.36 & 3.22e-03 & 8.44e-02 & 2.11e-02\\
 & 87GB194635.4+130713 & 0.30 & 2.67e-03 & 7.00e-02 & 1.75e-02\\
 & 87GB201926.8+061922 & 0.24 & 2.16e-03 & 5.66e-02 & 1.41e-02\\
\hline
& & \textbf{14.87} & \textbf{1.3e-01} &\textbf{3.5}  & \textbf{8.7e-01} \\
\hline
38& NONE & 0.0 & 0.0 & 0.0\\
\hline
& & \textbf{0.00} & \textbf{0.0e+00} &\textbf{0.0}  & \textbf{0.0e+00} \\
\hline
\end{tabular}
\end{table}
\begin{table}[b]\centering\fontsize{5.5}{5.7}\selectfont
\addtocounter{table}{-1}
\caption{contd.}
\begin{tabular}{llllll}

IC & Source & \#$\nu$ & \#$\nu_{\mathrm{emp.}}$ & \#$\nu_{\mathrm{scale, int.}}$ & \#$\nu_{\mathrm{f}}$\\
\hline
39 & PKS0727-11 & 16.79 & 1.49e-01 & 3.10e+00 & 7.76e-01\\
 & TXS0637-128 & 5.72 & 5.09e-02 & 1.06e+00 & 2.64e-01\\
 & PKS0646-306 & 3.97 & 3.54e-02 & 7.35e-01 & 1.84e-01\\
 & PMNJ0608-1520 & 3.86 & 3.43e-02 & 7.13e-01 & 1.78e-01\\
 & PKS0648-16 & 3.17 & 2.82e-02 & 5.86e-01 & 1.46e-01\\
 & PKS0627-199 & 3.06 & 2.72e-02 & 5.66e-01 & 1.41e-01\\
 & TXS0628-240 & 2.61 & 2.32e-02 & 4.82e-01 & 1.20e-01\\
 & TXS0745-165 & 2.01 & 1.79e-02 & 3.71e-01 & 9.28e-02\\
 & TXS0700-197 & 1.86 & 1.65e-02 & 3.44e-01 & 8.59e-02\\
 & NVSSJ062753-152003 & 1.78 & 1.59e-02 & 3.30e-01 & 8.24e-02\\
 & PMNJ0634-2335 & 1.61 & 1.43e-02 & 2.98e-01 & 7.44e-02\\
 & TXS0616-116 & 1.58 & 1.41e-02 & 2.93e-01 & 7.32e-02\\
 & 1RXSJ064444.2-285120 & 1.33 & 1.18e-02 & 2.46e-01 & 6.15e-02\\
 & PMNJ0618-2426 & 1.29 & 1.15e-02 & 2.39e-01 & 5.97e-02\\
 & 1RXSJ072259.5-073131 & 1.15 & 1.03e-02 & 2.13e-01 & 5.33e-02\\
 & TXS0646-176 & 1.14 & 1.02e-02 & 2.11e-01 & 5.27e-02\\
 & TXS0752-116 & 0.97 & 8.64e-03 & 1.80e-01 & 4.49e-02\\
 & PMNJ0622-2605 & 0.84 & 7.45e-03 & 1.55e-01 & 3.87e-02\\
 & CRATESJ061733.67-171522.8 & 0.65 & 5.77e-03 & 1.20e-01 & 3.00e-02\\
 & TXS0728-054 & 0.62 & 5.54e-03 & 1.15e-01 & 2.88e-02\\
 & 1RXSJ064933.8-313914 & 0.45 & 3.98e-03 & 8.27e-02 & 2.07e-02\\
\hline
& & \textbf{56.47} & \textbf{5.0e-01} &\textbf{10.4}  & \textbf{2.6e+00} \\
\hline
40 & MRC1036-529 & 7.38 & 6.57e-02 & 1.29e+00 & 3.22e-01\\
 & PMNJ0845-5458 & 3.89 & 3.47e-02 & 6.80e-01 & 1.70e-01\\
 & PMNJ0852-5755 & 3.85 & 3.42e-02 & 6.72e-01 & 1.68e-01\\
 & (PMNJ1006-5018) & 3.71 & 3.30e-02 & 6.48e-01 & 1.62e-01\\
 & PKS0903-57 & 3.31 & 2.95e-02 & 5.79e-01 & 1.45e-01\\
 & PKS0920-39 & 2.41 & 2.15e-02 & 4.21e-01 & 1.05e-01\\
 & PMNJ1022-4232 & 1.85 & 1.64e-02 & 3.23e-01 & 8.06e-02\\
 & PMNJ1014-4508 & 1.22 & 1.09e-02 & 2.13e-01 & 5.34e-02\\
 & RXJ1023.9-4336 & 0.79 & 7.02e-03 & 1.38e-01 & 3.45e-02\\
\hline
& & \textbf{28.41} & \textbf{2.5e-01} &\textbf{5.0}  & \textbf{1.2e+00} \\
\hline
45& NONE & 0.0 & 0.0 & 0.0\\
\hline
& & \textbf{0.00} & \textbf{0.0e+00} &\textbf{0.0}  & \textbf{0.0e+00} \\
\hline
46 & PKS1004-217 & 3.00 & 2.67e-02 & 5.26e-01 & 1.31e-01\\
 & PMNJ1008-2912 & 1.75 & 1.55e-02 & 3.06e-01 & 7.66e-02\\
 & 1RXSJ102658.5-174905 & 1.18 & 1.05e-02 & 2.07e-01 & 5.18e-02\\
 & NVSSJ103040-203032 & 0.88 & 7.80e-03 & 1.54e-01 & 3.84e-02\\
 & TXS0956-244 & 0.52 & 4.64e-03 & 9.15e-02 & 2.29e-02\\
 & TXS0936-173 & 0.50 & 4.47e-03 & 8.81e-02 & 2.20e-02\\
 & 1RXSJ094709.2-254056 & 0.37 & 3.31e-03 & 6.52e-02 & 1.63e-02\\
\hline
& & \textbf{8.20} & \textbf{7.3e-02} &\textbf{1.4}  & \textbf{3.6e-01} \\
\hline
48 & PKSB1424-328 & 3.47 & 3.09e-02 & 6.63e-01 & 1.66e-01\\
 & PMNJ1347-3750 & 2.08 & 1.85e-02 & 3.97e-01 & 9.93e-02\\
 & 1RXSJ144037.4-384658 & 1.95 & 1.74e-02 & 3.73e-01 & 9.34e-02\\
 & PKS1348-289 & 1.61 & 1.43e-02 & 3.07e-01 & 7.69e-02\\
 & NVSSJ134543-335643 & 1.49 & 1.33e-02 & 2.85e-01 & 7.12e-02\\
 & SUMSSJ135625-402820 & 1.46 & 1.30e-02 & 2.80e-01 & 7.00e-02\\
 & PKS1341-366 & 1.04 & 9.27e-03 & 1.99e-01 & 4.97e-02\\
 & PMNJ1359-3746 & 0.72 & 6.40e-03 & 1.37e-01 & 3.43e-02\\
 & NVSSJ134706-295840 & 0.64 & 5.70e-03 & 1.22e-01 & 3.06e-02\\
 & NVSSJ142750-321515 & 0.22 & 1.99e-03 & 4.26e-02 & 1.07e-02\\
\hline
& & \textbf{14.69} & \textbf{1.3e-01} &\textbf{2.8}  & \textbf{7.0e-01} \\
\hline
52 & PMNJ1648-4826 & 29.81 & 2.65e-01 & 5.23e+00 & 1.31e+00\\
 & PMNJ1650-5044 & 7.45 & 6.63e-02 & 1.31e+00 & 3.27e-01\\
 & PMNJ1717-5155 & 7.23 & 6.43e-02 & 1.27e+00 & 3.17e-01\\
 & AT20GJ164513-575122 & 7.05 & 6.28e-02 & 1.24e+00 & 3.10e-01\\
 & PMNJ1711-5028 & 6.12 & 5.44e-02 & 1.07e+00 & 2.69e-01\\
 & MRC1613-586 & 5.77 & 5.14e-02 & 1.01e+00 & 2.53e-01\\
 & PMNJ1723-5614 & 1.75 & 1.56e-02 & 3.07e-01 & 7.67e-02\\
\hline
& & \textbf{65.18} & \textbf{5.8e-01} &\textbf{11.4}  & \textbf{2.9e+00} \\
\hline
\hline
All & Total &492.50 & 4.38  & 96.52 & 24.13 \\
\hline
\end{tabular}
\end{table}

